Application of Sensitivity Analysis Methods for Studying Neural Network Models

This study demonstrates the capabilities of several methods for analyzing the sensitivity of neural networks to perturbations of the input data and interpreting their underlying mechanisms. The investigated approaches include the Sobol global sensitivity analysis, the local sensitivity method for input pixel perturbations and the activation maximization technique. As examples, in this study we consider a small feedforward neural network for analyzing an open tabular dataset of clinical diabetes data, as well as two classical convolutional architectures, VGG-16 and ResNet-18, which are widely used in image processing and classification. Utilization of the global sensitivity analysis allows us to identify the leading input parameters of the chosen tiny neural network and reduce their number without significant loss of the accuracy. As far as global sensitivity analysis is not applicable to larger models we try the local sensitivity analysis and activation maximization method in application to the convolutional neural networks. These methods show interesting patterns for the convolutional models solving the image classification problem. All in all, we compare the results of the activation maximization method with popular Grad-CAM technique in the context of ultrasound data analysis.

==> images/input/table1.tex <==
\begin{table}[H]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Pregnancies} & \textbf{Glucose} & \textbf{BloodPressure} & \textbf{SkinThickness} & \textbf{Insulin} & \textbf{BMI} & \textbf{DiabetesPedigreeFunction} & \textbf{Age} & \textbf{Outcome} \\ \midrule
6                   & 148              & 72                    & 35                     & 0               & 33.6         & 0.627                          & 50           & 1               \\
1                   & 85               & 66                    & 29                     & 0               & 26.6         & 0.351                          & 31           & 0               \\
8                   & 183              & 64                    & 0                      & 0               & 23.3         & 0.672                          & 32           & 1               \\
1                   & 89               & 66                    & 23                     & 94              & 28.1         & 0.167                          & 21           & 0               \\
0                   & 137              & 40                    & 35                     & 168             & 43.1         & 2.288                          & 33           & 1               \\
\vdots               & \vdots           & \vdots                & \vdots                  & \vdots           & \vdots       & \vdots                          & \vdots       & \vdots           \\ \bottomrule
\end{tabular}%
}
\caption{данные о диабете}
\end{table}


